Invasion Dynamics in the Biased Voter Process

The voter process is a classic stochastic process that models the invasion of a mutant trait $A$ (e.g., a new opinion, belief, legend, genetic mutation, magnetic spin) in a population of agents (e.g., people, genes, particles) who share a resident trait $B$, spread over the nodes of a graph. An agent may adopt the trait of one of its neighbors at any time, while the invasion bias $r\in(0,\infty)$ quantifies the stochastic preference towards ($r>1$) or against ($r<1$) adopting $A$ over $B$. Success is measured in terms of the fixation probability, i.e., the probability that eventually all agents have adopted the mutant trait $A$. In this paper we study the problem of fixation probability maximization under this model: given a budget $k$, find a set of $k$ agents to initiate the invasion that maximizes the fixation probability. We show that the problem is NP-hard for both $r>1$ and $r<1$, while the latter case is also inapproximable within any multiplicative factor. On the positive side, we show that when $r>1$, the optimization function is submodular and thus can be greedily approximated within a factor $1-1/e$. An experimental evaluation of some proposed heuristics corroborates our results.

==> sections/04.2.submodularity_bk.tex <==
\subsection{Monotonicity and Submodularity}\label{subsec:submodularity}

A real-valued set function~$f$ is called monotone if for any two sets~$A$ and~$B$ with~$A\subseteq B$, we have~$f(A)\leq f(B)$. Further, $f$ is called submodular if for all sets~$A$ and~$B$ we have
\[
f(A)+f(B)\geq f(A\cup B) + f(A\cap B) .
\numberthis\label{eq:submodularity}
\]
Monotone submodular functions, even if hard to maximize, admit efficient approximations. Here we complement the hardness of~\cref{thm:positive_bias_np_hard} 
by showing that~$\fp^G_{r \geq 1} (\SeedSet)$ is monotone and submodular. 
Although submodularity is well-known for some \emph{unidirectional} invasion processes~\cite{Kempe2003}, recall that our setting is \emph{bidirectional}, i.e., the mutant set may grow or shrink in any step. 
This bidirectionality renders submodularity a non-trivial property.


\Paragraph{Node duplication.
Towards establishing monotonicity and submodularity, it is convenient to view the process in a slightly different but equivalent way, via \emph{node duplication}. Consider the voter process~$\mathcal{M}$ on a graph~$G$ with bias~$r>1$. The node duplication view of~$\mathcal{M}$ is another stochastic process~$\mathcal{M}'=(\RandomConfiguration'_i)_i$ on~$G$, defined as follows. Let~$\Configuration\subseteq V$ be the current configuration.
\begin{compactenum}
\item A node~$u$ is chosen for death uniformly at random (i.e., this step is identical to~$\mathcal{M}$).
\item We modify~$G=(V,E,\Weight)$ to~$G'=(V',E', \Weight')$ as follows. For every node~$v \in \Neighbors(u) \cap \Configuration$, we create a duplicate~$v'$ of~$v$, and insert an edge~$(v',u)$ in~$G'$ with weight~$\Weight'(v',u) = \Weight(v,u)$. We associate~$v'$ with fitness~$\fit'_{\Configuration} (v') = r-1$, while every other node~$v\in V$ gets fitness $\fit'_{\Configuration}(v)=1$. % pk corrected from r-1 to 1.
Finally, we execute a stochastic birth step as in the standard voter process, i.e., we choose a node~$v$ to propagate to~$u$ with probability
\[
\frac{\fit'_{\Configuration}(v)\cdot \Weight'(v,u)}{\sum_{x}\fit'_{\Configuration}(x)\cdot \Weight'(x,u)}
\]
The new configuration~$\RandomConfiguration'_{i+1}$ contains~$u$ if either some mutant node~$v$ or its duplicate~$v'$ was chosen for reproduction. It is straightforward to see that this modified birth step preserves the probability distribution of random configurations, and thus~$\mathcal{M}$ and~$\mathcal{M}'$ are equivalent.
\end{compactenum}}

\paragraph{Monotonicity.} Using the equivalence between the voter process and its variant with node duplication, we now establish the monotonicity of the fixation probability.

\begin{restatable}{lemma}{lemmonotonicity}\label{lem:monotonicity}
For any graph~$G$ and bias~$r$, for any two seed sets~$\SeedSet_1$ and~$\SeedSet_2$ with~$\SeedSet_1 \subseteq \SeedSet_2$, we have~$\fp^G_{r}(\SeedSet_1) \leq \fp^G_{r}(\SeedSet_2)$.
\end{restatable}
\begin{myproof}
First assume~$r>1$. Consider two processes~$\mathcal{M}_1=(\RandomConfiguration^1_i)_i$ and~$\mathcal{M}_2 = (\RandomConfiguration^2_i)_i$ starting from~$\RandomConfiguration^1_0 = \SeedSet_1$ and~$\RandomConfiguration^2_0 = \SeedSet_2$, respectively. We establish a coupling between~$\mathcal{M}_1$ and~$\mathcal{M}_2$ that satisfies~$\RandomConfiguration^1_i \subseteq  \RandomConfiguration^2_i$ for all~$i\geq 0$, from which the lemma follows.

In each step, we first choose the same node~$u$ for death in $\mathcal{M}_2$ and~$\mathcal{M}_1$ with uniform probability. 
Then, we execute a birth step in~$\mathcal{M}_2$. 
If the reproducing node~$v$ is present in~$\mathcal{M}_1$, we perform the same update in~$\mathcal{M}_1$. 
Otherwise, if~$v$ is a mutant duplicate absent from~$\mathcal{M}_1$, we perform an independent birth step in~$\mathcal{M}_1$. 
This coupling maintains the invariant~$\RandomConfiguration^1_i \subseteq \RandomConfiguration^2_i$, as whenever~$\mathcal{M}_1$ takes an independent step, a mutant has reproduced in~$\mathcal{M}_2$. Moreover, the coupling is indeed transparent to~$\mathcal{M}_1$ and~$\mathcal{M}_2$, as every birth event occurs with probability proportional to its agent's fitness.

The monotonicity for all~$r$ follows by symmetry, as when~$r<1$ we can exchange the roles of mutants and residents. Using the above argument, it follows that the fixation probability of the residents grows monotonically in~$V\setminus \SeedSet$ and, in reverse, decreases monotonically as~$V \setminus \SeedSet$ shrinks, hence the fixation probability of the mutants grows monotonically in~$\SeedSet$.
\end{myproof}

\Paragraph{Submodularity.} 
We now show submodularity, i.e., we have
\[
\fp^G_{r}(A)+\fp^G_{r}(B)\geq \fp^G_{r}(A\cup B) + \fp^G_{r}(A\cap B) .
\numberthis\label{eq:submodularity_fp}
\]
To this end, it is convenient to consider the following more refined view of the invasion process. Given an initial seed set~$\SeedSet=A\cup B$, we keep track not only of the mutant set, but also the subset of mutants that are copies of the agents initially in~$A \setminus B$. Consider this refined view, and execute the invasion beyond the point where mutants fixate. With probability~1, we eventually reach a configuration in which \emph{all} mutants are copies of either~$A$ or~$B$. In this case, we say that~$A$ (resp., $B$) has fixated; with a small abuse of notation, we write~$\fp^G_{r}(\SeedSet, A)$ (resp., $\fp^G_{r}(\SeedSet, B)$) for the probability of that event. Thus~$\fp^G_{r}(\SeedSet) = \fp^G_{r}(\SeedSet, \SeedSet)$, and it follows that
\[
\fp^G_{r}(A\cup B, A\cup B) = \fp^G_{r}(A\cup B, A) + \fp^G_{r}(A\cup B,B)
\numberthis\label{eq:additive}
\]
as a fixation of either~$A$ or~$B$ implies that of~$A\cup B$ and, in reverse, a fixation of~$A\cup B$ eventually leads to that of either~$A$ or~$B$. \cref{eq:additive} is instrumental in proving submodularity.

\begin{restatable}{lemma}{lemsubmodular}\label{lem:submodular}
For any graph~$G$ and bias~$r\geq 1$, the fixation probability~$\fp^G_{r}(\SeedSet)$ is submodular.
\end{restatable}
\begin{myproof}
Consider any two sets~$A,B\subseteq V$. Let~$\mathcal{M}_1$, $\mathcal{M}_2$, $\mathcal{M}_3$ and~$\mathcal{M}_4$ be the four invasion processes, under node duplication, that correspond to initial seeds~$A$, $B$, $A\cup B$ and~$A\cap B$, respectively. For~$j\in [4]$, let~$\RandomConfiguration^j_i$ be the~$i$-th random configuration of~$\mathcal{M}_j$. Moreover, let~$\RandomYConfiguration_i$ (resp., $\RandomZConfiguration_i$) be the set of nodes of $\mathcal{M}_3$ in step~$i$  that are occupied by mutant agents  who are descendants of some agent initially in~$A$ (resp., $B$). We establish a four-way coupling between all~$\mathcal{M}_j$ that preserves the following invariants:
\[
\text{(i)}~\RandomYConfiguration_i\subseteq \RandomConfiguration^1_i
\qquad
\text{(ii)}~\RandomZConfiguration_i\subseteq \RandomConfiguration^2_i
\quad
\text{and}
\quad
\text{(iii)}~\RandomConfiguration^4_i\subseteq \RandomConfiguration^1_i\cap \RandomConfiguration^2_i .
\]
Due to \cref{eq:additive}, invariants (i) and (ii) guarantee that any fixating run in~$\mathcal{M}_3$ is also fixating in at least one of~$\mathcal{M}_1$ and~$\mathcal{M}_2$ with at least as large probability. Invariant (iii) guarantees that any fixating run in~$\mathcal{M}_4$ is fixating in both~$\mathcal{M}_1$ and~$\mathcal{M}_2$, each of the latter having at least as large probability. Hence, the three invariants imply \cref{eq:submodularity_fp}, i.e., submodularity.

We now establish the coupling. In each step~$i$, we choose the same node~$u$ in all~$\mathcal{M}_j$ to die uniformly at random. Then, as long as~$\RandomYConfiguration_i,\RandomZConfiguration_i \neq \emptyset$ we perform the following steps.
\begin{compactenum}
\item Choose a node~$v$ to reproduce in~$\mathcal{M}_3$ using node duplication (hence~$v$ is either an original or a duplicate node). For each process~$\mathcal{M}_j$ in which~$v$ is a node (either original or duplicate), propagate the agent from~$v$ to~$u$. Note that this step updates~$\mathcal{M}_3$ and at least one of~$\mathcal{M}_1$ and~$\mathcal{M}_2$, while if it updates~$\mathcal{M}_4$, it also updates both~$\mathcal{M}_1$ and~$\mathcal{M}_2$.
\item If~$v$ is not a node in one of~$\mathcal{M}_1$ or~$\mathcal{M}_2$, then perform an independent birth step in that process, choosing some node~$x$ (either original or duplicate). If~$x$ is present in~$\mathcal{M}_4$, apply the birth event in~$\mathcal{M}_4$ as well, otherwise apply an independent birth step in~$\mathcal{M}_4$.
\end{compactenum}

If $\RandomYConfiguration_i= \emptyset$ or $\RandomZConfiguration_i= \emptyset$, we perform step~2 only in the process not yet terminated. 
As in~\cref{lem:monotonicity}, the coupling is indeed transparent to each~$\mathcal{M}_j$ and maintains invariants~(i)--(iii).
\end{myproof}

Conclusively, monotonicity and submodularity lead to the following approximation guarantee~\cite{Nemhauser1978}.

\begin{restatable}{theorem}{thmpositivebiasapprox}\label{thm:positive_bias_approx}
Given a graph~$G$ and integer~$k$, let~$S^*$  be the seed set that maximizes~$\fp^G_{r}(\SeedSet)$,
and~$S'$ the seed set constructed by a greedy algorithm opting for maximal returns in each step. Then~$\fp^G_{r} (\SeedSet') \geq \left(1-\sfrac{1}{e}\right)\fp^G_{r}(\SeedSet^*)$.
\end{restatable}
